Zero-shot Policy Learning with Spatial Temporal RewardDecomposition on Contingency-aware Observation

It is a long-standing challenge to enable an intelligent agent to learn in one environment and generalize to an unseen environment without further data collection and finetuning. In this paper, we consider a zero shot generalization problem setup that complies with biological intelligent agents' learning and generalization processes. The agent is first presented with previous experiences in the training environment, along with task description in the form of trajectory-level sparse rewards. Later when it is placed in the new testing environment, it is asked to perform the task without any interaction with the testing environment. We find this setting natural for biological creatures and at the same time, challenging for previous methods. Behavior cloning, state-of-art RL along with other zero-shot learning methods perform poorly on this benchmark. Given a set of experiences in the training environment, our method learns a neural function that decomposes the sparse reward into particular regions in a contingency-aware observation as a per step reward. Based on such decomposed rewards, we further learn a dynamics model and use Model Predictive Control (MPC) to obtain a policy. Since the rewards are decomposed to finer-granularity observations, they are naturally generalizable to new environments that are composed of similar basic elements. We demonstrate our method on a wide range of environments, including a classic video game -- Super Mario Bros, as well as a robotic continuous control task. Please refer to the project page for more visualized results.

==> experiment_old.tex <==
\section{Experiment}\label{sec:exp}

In this section, we study how well our SAP framework performs compare to baselines, and the roles of various components in the framework. We conduct experiments on three domains: a didactic gridworld task, a famous video game ``Super Mario Bros''~\citep{gym-super-mario-bros} and a robotics blocked reacher task~\citep{huang2019mapping}. Environment details, architectures, hyper-parameters are described thoroughly in Appendix~\ref{appendix:specs}.

\subsection*{Didactic Example: Hidden Reward Gridworld}
\label{sec:grid}

\begin{figure*}
     \centering
     \begin{subfigure}{0.36\textwidth}
         \centering
         \includegraphics[width=\textwidth]{./contents/Fig/grid.pdf}
         \caption{Hidden Reward Gridworld Env}
         \label{fig:grid}
     \end{subfigure} 
     \rulesep
     \hfill
     \begin{subfigure}{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{./contents/exp_figs/main_reb.png}
         \caption{Mario train world returns}
         \label{fig:main} 
     \end{subfigure}%
     \hfill
     \begin{subfigure}{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{./contents/exp_figs/generalization_reb.png}
         \caption{Mario test world returns}
         \label{fig:generalization}
     \end{subfigure}
        \caption{(a) The hidden reward gridworld example. See Section \ref{sec:grid} for more details. (b) \& (c) The total returns of different methods on the Super Mario Bros. %All the experiments are run with 50000 game steps on multiple episodes. 
        Error bars are shown as 95\% confidence interval. %except for the given interaction data. 
        See Section \ref{sec:comparisons} for details. \label{fig:full} %Best view in color.
        }
        \label{fig:three graphs}
        \vskip -0.5cm
\end{figure*}
To investigate whether the proposed framework can learn meaningful scores and hence induce correct policy, we start with a simple didactic task Hidden Reward Gridworld. 
%where the environment matches the assumptions of our method. 
%This environment will reveal to what level can our method recover the per step scores.
%\vspace{-0.55 pt}
Figure \ref{fig:full}\subref{fig:grid} shows an illustrative example of the Hidden Reward Gridworld. In the grid world, there is an object at each location, where each type of object is associated with an unknown number. The agent has explored random trajectories, with the knowledge of sum of numbers along each trajectory.

\begin{wraptable}{R}[True]{0.55\textwidth}
{\small
\centering
\caption{\label{table:didactic}The average error for the learned object points and the total returns. See Sec. \ref{sec:grid_table_analysis} for analysis. }
\begin{tabular}{@{}lrrcrrr@{}}\toprule
& \multicolumn{2}{c}{World 1} & \phantom{ab}& \multicolumn{2}{c}{World 2} &
\phantom{ab} \\
\cmidrule{2-4} \cmidrule{5-7} 
           & error  & returns && error & returns \\ \midrule
SAP      & 0.04 & \textbf{378.6} && 0.34 &  \textbf{389.8}\\
BC-random & - & 83.05  && -  &  106.8 \\
BC-SAP & - & 333  && -  &  300.0 \\
\bottomrule
\end{tabular}
}
\vskip -0.3cm
\end{wraptable}

%It needs to learn the value of each object and collect as much value as possible in a new environment with different object configurations. In our experiment, we use an $8 \times 8$ grid, with 16 different types of objects, and each of them worth a value of 0, 1 to 15 respectively. 
To make the task more challenging, instead of giving the identity of each object by object id, we are using a 16-dimensional noisy feature to mimic the output of a perception network from visual inputs. For the testing environment (World 2), we use different configuration, with the same feature vectors and new Gaussian noise.
\label{sec:grid_table_analysis}
%On this task, our method operates as follows. 
%We use a two layer fully connected neural network to predict per step score from the 16-dimensional feature. Those per step scores are aggregated by a sum operator, and fitted to the training data. We opt to use the environment dynamics model, because it can be perfectly learned by a tabular function. 
% \begin{table}

% \end{table}
As shown in Table~\ref{table:didactic}, we find that a neural network can fit the object value based on the features with an error 0.04 on a training environment and 0.34 on a new task even with the feature noise presence. To see how well our method performs on this task, we train two behavior cloning agents: an agent imitates the exploratory data (denoted as BC-random) and the other imitates the behavior of a fully trained SAP on the training environment (denoted as BC-SAP). As shown in Table~\ref{table:didactic}, BC-random has far inferior performance, since it clones the exploration behavior. BC-SAP perform inferior to our method, especially in the test world. This shows that even allowed to clone the behavior of SAP, behavior cloning still does not generalize as well as our method in a new environment. We have shown that SAP is capable of learning accurate scoring functions, in the face of object feature noises.

%In this grid world environment, we have shown that SAP is capable of learning accurate scoring functions, even in the presence of object feature noises. We have also demonstrated that SAP would generalize better than alternative algorithms. 


\subsection{SAP on Super Mario Bros with sparse rewards}
To evaluate our proposed algorithm in a more realistic environment, we run SAP and a few alternative methods in the Super Mario Bros environment. In this environment, we neither have a clear definition of the dense score for each step, nor the aggregation procedure. This environment also features high-dimensional visual observations, which is more challenging since we have a larger hypothesis space.  The original game has 240 $\times$ 256 image input and discrete action space with 5 choices. We wrap the environment following \citet{mnih2015human} and what described in Appendix~\ref{sec:mario_app}; finally, we obtain a $84 \times 84$ size 4-frame gray-scale stacked observation. The goal for an agent is to survive and go toward the right as far as possible. The environment returns how far the agent goes to the right at the end of a trajectory as the delayed terminal sparse reward. Please see Appendix~\ref{sec:mario_app} for details. 


\subsubsection{Comparisons}
\label{sec:comparisons}
We compare our method with the various baselines including exploration data, behavior cloning~\cite{pomerleau1989alvinn, bain1995framework}, model based with Human Prior where the prior is specified manually, DARLA~\citep{higgins2017darla}, RUDDER~\cite{arjona2018rudder}, behavioral cloning with privilege data (imitating a bank of higher quality data), RL with curiosity. We note that although the baselines BC with privilege data and RL with curiosity needs extra environmental steps or other data, SAP still outperform them. Please see Appendix~\ref{sec:mario_baseline_app} for thorough description and implementation details. 


%\begin{table}[h]
\begin{wraptable}{R}[True]{0.55\textwidth}
{\small
\centering
\caption{Components Ablations. The averaged return is reported.  95\% confidence interval is shown in the bracket. Higher is better. S, A, P represent the Scoring, Aggregating and Planning parts respectively. \label{table:md}}
\begin{tabular}{@{}llllll@{}}\toprule
            & {S} & {A} & {P} & W1S1(train)&W2S1(test)
            \\ \midrule
SAP           &  yes    & yes  & yes     & \textbf{1359.3[68.5]} & \textbf{790.1[35.7]} \\
MBHP           &  no & no   & yes     & 1041.3[149.0] & 587.8[31.0]  \\
SAP-3   &  yes    & yes  & less & 944.5[133.5]  & 444.3[14.7]   \\
Greedy        &  yes    & yes  & no      & 302.0[27.9]  & 40.0[15.7] \\
\bottomrule
\end{tabular}
}
%\vskip -0.3cm
\end{wraptable}

%\end{table}
\textbf{Analysis} Fig.~\ref{fig:three graphs}~\subref{fig:main} and Fig.~\ref{fig:three graphs}~\subref{fig:generalization} show how the above methods performs in the Super Mario Bros. The \texttt{Explore} baseline shows the average training trajectory performance. We found that \texttt{RUDDER} fails to match the demonstration performance. This is becaused the LSTM in RUDDER does not have sufficient supervision signals from the long term delayed rewards in the Mario environment. \texttt{DARLA} slightly outperforms the demonstration data in training. Its performance is limited by the unsupervised visual disentangled learning step, which is a hard problem in the complex image domain. \texttt{Behavior Cloning} is slightly better than the exploration data, but much worse than our method. \texttt{MBHP} is a model-based approach where human defines the scoring function. Human priors are usually hard to get. In this task, it is inferior to SAP's learned priors. We further compare to two methods that utilize privileged information. The \texttt{Privileged BC} method trains on near optimal data, and performs quite well during training; however, it performs much worse during the zero shot testing. The similar trend happens with \texttt{RL Curiosity}, which has the privileged access to online interactions in the training environment. Those two methods shows that SAP even outperforms methods with privileged data in the zero shot condition. 

%\textbf{Analysis} In Figure.~\ref{fig:full}\subref{fig:main}, the results show that the proposed SAP model outperforms all the baselines with a large margin on the same level they are trained on. We believe that there are two major reasons for BC's unsatisfactory performance: 1. we only have access to the exploration data which is suboptimal for the task. 2. When seeing rare events in the game (the exploration data hardly reach the ending part), it fails to generalize. SAP also outperforms DARLA on both training and generalization tasks. We believe it is because observations can change dramatically between train and test levels. Thus, DARLA's learned disentangled representations can't generalize well enough in test level. Comparing the SAP model with the MBHP method, we demonstrate the learned priors can empower an agent with a better understanding of the world thus stronger performance. We believe rudder fails on the environment for two reasons: 1. Rudder is trained on 
%We show qualitative results in the subsection~\ref{sec:viz} to validate that the learned priors contain meaningful scores that leads to better actions. SAP also outperforms all the baselines in an unseen level without any finetuning (Fig.~\ref{fig:full}\subref{fig:generalization}), which proves that it can generalize well. \bibiY{There should be more convincing reasons that explains why our method is better than the DARLA and rudder baselines}


\subsubsection{Ablative Studies}
\label{sec:ablation}
In order to understand why SAP framework, we conduct three sets of ablative studies in this section. %In the first set of ablations, we ablate each factor of a full SAP framework. In the second set, we compare SAP to two oracle methods to test its generalization capability. 

\textbf{Components Ablations}
In order to understand why SAP achieves superior performances, we ablate components of SAP. In Table~\ref{table:md}, we list 4 methods: the full SAP method, the SAP without scoring and aggregating (MBHP), the SAP method with fewer (3) planning steps (SAP-3), the SAP method without the planning part (Greedy). We observe that the performance drops significantly if turning off any of those components, which shows the importance of all components. %The biggest drop happens when there is no planning part. We can see that the planning part is vital to the performance, especially the generalization, and the scoring part is also crucial to the performance. 





\textbf{Scoring Function Ablations}
The SAP framework allow us to flexibly choose the scoring function. In this section, we investigate the empirical difference between a simple scoring function versus a structured one. As we discussed in Section~\ref{sec:score_design}, a simple scoring function refers to a CNN which takes in the egocentric state and output the action-conditioned score. A structured scoring function further divide the egocentric state into several sub-regions, and reuse the same CNN to predict the score. Please see Appendix~\ref{sec:app:mario_arch} for details. 

As shown in Table~\ref{table:visual_representation}, we find a more structured scoring function can further enhance the empirical performance upon a simple one, likely due to parameter sharing; moreover, even the simple scoring function with SAP outperforms all the other methods in the Super Mario Bros experiment. This effectively shows that it is the SAP framework, rather than the specific design of the scoring function that results in the superior performance. 
\begin{wraptable}{R}[True]{0.45\textwidth}
{\small
\centering
\caption{Ablation study of the scoring function. The averaged return is reported. We only show MBHP, which is the best performing method among previous approaches. \label{table:visual_representation}}
\begin{tabular}{@{}lll@{}}\toprule
& {W1S1(train)} & {W2S1(test)} 
            \\ \midrule
SAP-structured score      & \textbf{1359.3} & \textbf{790.1}  \\
SAP-simple score     & 1258.0          & 737.0  \\
MBHP                 & 1041.3          & 587.9  \\
\bottomrule
\end{tabular}
\vskip -0.3cm
}
\end{wraptable}

\textbf{Egocentric Observation Ablation} SAP utilizes egocentric observation instead of global observation to learn the scores. To make sure egocentric observation does not make the problem simpler, we ablate the observation space with the behavior cloning method. We found that BC with global observation performs better that BC with egocentric observation in the training environment, but their performance during test is almost the same. This shows that, with the same algorithm, the egocentric observation does not make the generalization task easier.

\textbf{Perfect Dynamics and No Done Signal}
Towards understanding the effect of different components of SAP, we investigate the performance of an agent using learned scores on a perfect dynamics model which shows the upper bound for improvement from better models. In Fig.~\ref{fig:ablation}\subref{fig:ablation_c}, we found that both MBHP and SAP benefit from the perfect dynamics a lot. This suggests that SAP can perform much better if future techniques can develop a better dynamics model. 
\begin{wraptable}{R}[True]{0.55\textwidth}
{\small
\centering
\caption{Ablation of the egocentric observation space versus the global observation space. \label{table:ablate_obs}}
\begin{tabular}{@{}lll@{}}\toprule
& {World 1 Stage 1} & {World 2 Stage 1} 
            \\ \midrule
BC-global obs      & \textbf{961.1}[59.4] & \textbf{455.4}[18.4]  \\
BC-egocentric obs     & 822.5[44.9]          & \textbf{457.3}[20.0]  \\
\bottomrule
\end{tabular}
\vskip -0.3cm
}
\end{wraptable}

\label{sec:mario_ablation}
\begin{figure}[h]
\centering
\begin{subfigure}{0.31\linewidth}
   \centering
   \includegraphics[width=\linewidth]{./contents/exp_figs/gen_perfect.png}
   \caption{GT dynamics model          on W2S1 (test)}
   \label{fig:ablation_c} 
\end{subfigure}
\hfill
\begin{subfigure}{0.31\linewidth}
   \centering
   \includegraphics[width=\linewidth]{./contents/exp_figs/gen_nodeath_per.png}
   \caption{GT dynamics model \& no done on W2S1 (test)}
   \label{fig:ablation_d}
\end{subfigure}
\hfill
\begin{subfigure}{0.31\linewidth}
%\begin{figure}
   \centering
   \includegraphics[width=\linewidth]{./contents/visualization/viz_5_1.png}
\caption{{\small Visualized greedy actions from the learned scores in a new level (W5S1).}}\label{fig:viz}
\vskip -0.3cm
%\end{figure}
\end{subfigure}

\caption{(a) is SAP with the groundtruth oracle dynamics model, (b) is similar to (a) but without the true ``done'' signal. Error bar is 95\% confidence interval.} \label{fig:ablation}
\vskip -0.3cm
\end{figure}

We hypothesize that the ``done'' signal from the perfect model contributes to the superior performance because it naturally tells an MPC algorithm not to select a short trajectory if reward at every step is positive (e.g. in the MBHP). In Fig.~\ref{fig:ablation}\subref{fig:ablation_d}, we see that if ``done'' signal is not provided, SAP still preserves the performance and outperforms all the baselines. However, we find MBHP significantly dropped below the level of exploration data return.
\color{black} More ablation studies, such as planning horizon, please refer to Appendix~\ref{sec:mario_ablation_app}. 


\subsubsection{Visualization of learned scores}\label{sec:viz}
In this section, we qualitatively study the induced action by greedily maximizing one-step score. %The actions can be suboptimal and different from the policy described above because the greedy actions only consider one-step score but it still capture the behavior of a policy.
We visualize the computed actions on World 5 Stage 1 (Figure.~\ref{fig:viz}) which is visually different from previous tasks. In this testing case, we see that the actions are reasonable, such as avoiding obstacles and monsters by jumping over them, even in the face of previously unseen configurations and different backgrounds. However, the ``Piranha Plants'' are not recognized because all the prior scores are learned from W1S1 where it never appears. More visualization of action maps is available in Appx.~\ref{sec:mario_viz_app} and Appx.~\ref{sec:mario_viz_app}, Fig.~\ref{fig:viz_score}. Those qualitative studies further demonstrate that the SAP method can assign meaningful scores for different objects in an unsupervised manner. 
It also produces good actions even in a new environment. 
%Additionally, we visualize the prior scores for different representative local sub-regions in Appendix~\ref{sec:mario_viz_app}, Figure.~\ref{fig:viz_score}. In this setting, we synthetically put an agent on a different relative position near an object. We find that our method learns meaningful scores such as assigning low scores for walking towards ``koopa''(turtle) and a high score for jumping. 


%In Fig.~\ref{}, we apply the learned score function to an image sampled from the game. The score map is added to the original image as an alpha channel. The ``sky'' and ``ground'' generally has a small positive value while the monsters ``goomba'' and ``koopa'' have a larger negative value. Also, the green tube has a negative value because it can block the agent from going to the right.


\subsection{SAP on the 3-D robotics task}
\begin{wraptable}{R}[True]{0.55\textwidth}
{
    \small
    \centering
    \caption{{\small Evaluation of SAP, MBHP and Rudder on the 3D Reacher environment. Numbers are the avg. steps to reach the goal. The lower the better. Numbers in the brackets are the 95\% confidence interval. ``L'' denotes the learned dynamics, and ``P'' denotes the perfect dynamics.}}
    \label{tab:robot}
    \begin{tabular}{l@{\hspace{0.1cm}}c@{\hspace{0.2cm}}c@{\hspace{0.2cm}}c@{\hspace{0.2cm}}l}
        \toprule
        &Config A&Config B&Config C& Config D\\ \hline
        SAP(L)&\textbf{97.53}[2.5]&\textbf{86.53}[1.9]&\textbf{113.3}[3.0]&\textbf{109.2}[3.0]\\
        MBHP(L)&124.2[4.5]&102.0[3.0]&160.7[7.9]&155.4[7.2]\\
        Rudder(L)&1852[198]&1901[132]&1933[148]&2000[0.0]\\
        \hline
        SAP(P)&\textbf{97.60}[2.6]&\textbf{85.38}[1.8]&\textbf{112.2}[3.1]&\textbf{114.1}[3.2]\\
        MBHP(P)&125.3[4.3]&102.4[3.0]&153.4[5.3]&144.9[4.8]\\
        Rudder(P)&213.6[4.2]&194.2[7.0]&208.2[5.6]&201.5[6.3]
        \bottomrule
    \end{tabular}
    \label{tb:3d}
        % \vskip -0.3cm
}
\end{wraptable}

\label{sec:3d}
In this section, we further study the SAP method to understand its property with a higher dimensional observation space. We conduct experiments in a 3-D robotics environment, BlockedReacher-v0. In this environment, a robot hand is initialized at the left side of a table and tries to reach the right. Between the robot hand and the goal, there are a few blocks standing as obstacles. The task is moving the robot hand to reach a point on $y=1.0$ as fast as possible. To test the generalization capability, we create four different configurations of the obstacles, as shown in Figure~\ref{fig:samples}. Figure~\ref{fig:samples} A is the environment where we collect exploration data from and Figure~\ref{fig:samples}~B, C, D are the testing environments. Note that the exploration data has varying quality, where many of the trajectories are blocked by the obstacles. Please see Appendix~\ref{sec:app:sap_robot}

% \begin{table}[h]
%     \begin{minipage}[b]{0.6\linewidth}
%         \centering
%         \caption{Evaluation of SAP, MBHP and Rudder on the 3D Reacher environment. Numbers are 
%         the avg. steps to reach the goal. The lower the better. Numbers in the brackets are the 95\% confidence interval. ``L'' denotes the learned dynamics, and ``P'' denotes the perfect dynamics.}
%         \label{tab:robot}
%         \begin{tabular}{l@{\hspace{0.1cm}}c@{\hspace{0.2cm}}c@{\hspace{0.2cm}}c@{\hspace{0.2cm}}l}
%         \toprule
%         &Config A&Config B&Config C& Config D\\ \hline
%         SAP(L)&\textbf{97.53}[2.5]&\textbf{86.53}[1.9]&\textbf{113.3}[3.0]&\textbf{109.2}[3.0]\\
%         MBHP(L)&124.2[4.5]&102.0[3.0]&160.7[7.9]&155.4[7.2]\\
%         Rudder(L)&1852[198]&1901[132]&1933[148]&2000[0.0]\\
%         \hline
%         SAP(P)&\textbf{97.60}[2.6]&\textbf{85.38}[1.8]&\textbf{112.2}[3.1]&\textbf{114.1}[3.2]\\
%         MBHP(P)&125.3[4.3]&102.4[3.0]&153.4[5.3]&144.9[4.8]\\
%         Rudder(P)&213.6[4.2]&194.2[7.0]&208.2[5.6]&201.5[6.3]
%         \bottomrule
%         \end{tabular}
%         \label{tb:3d}
%         % \vskip -0.3cm
%     \end{minipage}\hfill
%     \begin{minipage}[b]{0.35\linewidth}
%         \centering
%         \includegraphics[width=0.8\linewidth]{contents/env_sample/task_composed.png}
%         \captionof{figure}{Four variants of the 3D robot reacher environments. See Section \ref{sec:3d} for details.}
%         \label{fig:samples}
%         \vskip -0.3cm
%     \end{minipage}
% \end{table}


% \begin{wrapfigure}{H}{0.36\linewidth}
% \centering
%   \begin{subfigure}{0.48\linewidth}
%   \centering
%   \includegraphics[width=\linewidth]{./contents/env_sample/task_0}
%   \caption{}\label{fig:robot0} 
% \end{subfigure}
% \hfill
% \begin{subfigure}{0.48\linewidth}
%   \centering
%   \includegraphics[width=\linewidth]{./contents/env_sample/task_1}
%   \caption{}\label{fig:robot1}
% \end{subfigure}
% \hfill
% \begin{subfigure}{0.48\linewidth}
%   \centering
%   \includegraphics[width=\linewidth]{./contents/env_sample/task_2}
%   \caption{}\label{fig:robot2} 
% \end{subfigure}
% \hfill
% \begin{subfigure}{0.48\linewidth}
%   \centering
%   \includegraphics[width=\linewidth]{./contents/env_sample/task_3}
%   \caption{}\label{fig:robot3} 
% \end{subfigure}
% \caption{Four variants of the 3D robot reacher environments. See Section \ref{sec:3d} for details.}\label{fig:samples}
% \vskip -0.3cm
% \end{wrapfigure}
\begin{wrapfigure}{R}{0.32\linewidth}
\centering
\includegraphics[width=\linewidth]{contents/env_sample/task_composed.png}
\caption{Four variants of the 3D robot reacher environments. See Section \ref{sec:3d} for details.}\label{fig:samples}
% \vskip -0.3cm
\end{wrapfigure}
We evaluate similar baselines as in the previous section that is detailed in Appendix~\ref{sec:robo_baseline_app}. In Table~\ref{tb:3d}, we compare our method with the MBHP and RUDDER on the 3D robot reaching task. We found that our method needs significantly fewer steps than the two baselines, in both training environment and testing ones. We find that SAP significantly moves faster to the right because it learns a negative score for crashing into the obstacles. However, the MBHP method, which has +1 positive for each 1 meter moved to the right, would be stuck by the obstacles for a longer duration. In RUDDER with perfect dynamics baseline, the arm also frequently waste time by getting stuck at obstacle. The case is more extreme in RUDDER with learned dynamics, where the arm is almost always blocked until maximum step. We found that our SAP model is relatively insensitive to the errors in the learned dynamics, such that the performance using the learned dynamics is close to that of perfect dynamics. These experiments show that our method can be applied to robotics environment that can be hard for some algorithms due to the 3-D nature. %Moreover, we demonstrate again that the SAP method perform much better than all other methods. %Moreover, we demonstrate again that using partial states (egocentric regions) with SAP generalize better than baselines. 




